Marginalization Consistent Probabilistic Forecasting of Irregular Time Series via Mixture of Separable flows

Probabilistic forecasting models for joint distributions of targets in irregular time series with missing values are a heavily under-researched area in machine learning, with, to the best of our knowledge, only two Models have been researched so far: The Gaussian Process Regression model, and ProFITi. While ProFITi, thanks to using multivariate normalizing flows, is very expressive, leading to better predictive performance, it suffers from marginalization inconsistency: It does not guarantee that the marginal distributions of a subset of variables in its predictive distributions coincide with the directly predicted distributions of these variables. When asked to directly predict marginal distributions, they are often vastly inaccurate. We propose MOSES (Marginalization Consistent Mixture of Separable Flows), a model that parametrizes a stochastic process through a mixture of several latent multivariate Gaussian Processes combined with separable univariate Normalizing Flows. In particular, MOSES can be analytically marginalized, allowing it to directly answer a wider range of probabilistic queries than most competitors. Experiments on four datasets show that MOSES achieves both accurate joint and marginal predictions, surpassing all other marginalization consistent baselines, while only trailing slightly behind ProFITi in joint prediction, but vastly superior when predicting marginal distributions.

==> contents/MI_metric.tex <==
\section{Measuring Marginalization Consistency Violation}\label{sec:mi_metric}


We assess how well a model's predicted marginals match those derived from its joint distribution using the \textbf{Wasserstein distance (WD)}.

For each variable $y_k$, we compare:
\begin{itemize}
	\item $\hat{p}(y_k \mid Q_k, X)$: the predicted marginal,
	\item $\hat{p}^\mar(y_k \mid Q_k, X)$: the marginal obtained by integrating the joint $\hat{p}(y \mid Q, X)$.
\end{itemize}

Since direct sampling from $\hat{p}^\mar$ is difficult, we sample from the joint and extract the $k$-th component.

The marginalization inconsistency is defined as the average WD across all $K$ variables:
\begin{align}
	\MI = \frac{1}{K} \sum_{k=1}^{K} \text{WD}_r\left( \hat{p}(y_k \mid Q_k, X), \hat{p}^\mar(y_k \mid Q_k, X) \right)
\end{align}

We use $r = 2$ and approximate using 1000 samples. Currently, we only use univariate marginals to assess marginalization inconsistency. In principle, multivariate marginals could also be used, however they are computationally prohibitively expensive due to a lack of a closed form solution for the WD as in \eqref{eq:wd_empirical}.


%To measure the marginalization inconsistency in a probabilistic model, we use the \textbf{Wasserstein distance} (WD) between the two distributions:
%\begin{enumerate}
%	\item Univariate marginals directly predicted by the model
%	\item Univariate marginals obtained from numerically integrating the joint distribution
%\end{enumerate}
%%
%corresponding to the left and right-hand side of~\eqref{eq:mar_consistency}.
%The Wasserstein $r$-distance between two univariate empirical distributions, $p_U^\emp$ and $p_V^\emp$, given by the samples $U=(u_1, \ldots, u_N)$ and $V=(v_1, \ldots, v_N)$, can be expressed in terms of the order statistics: \citep{bobkov_2019_one-dimensional_empirical_measures}
%%
%\begin{align}\label{eq:wd_empirical}
%	\text{WD}_r(p_U^\emp, p_V^\emp) = \Bigl(\frac{1}{N}\sum_{n=1}^{N} \Vert u_{\pi_n} - v_{\tau_n} \Vert^r \Bigr)^{1/r}
%\end{align}
%%
%here $\pi$ and $\tau$ are the permutations that sort the samples $U$ and $V$ respectively.
%
%For models $\hat{p}$ that can predict both:
%	(i) The univariate marginals $\hat{p}(y_k \mid Q_k, X)$, for $k = 1, \ldots, K$,
%	(ii) The joint distribution $\hat{p}(y \mid Q, X)$,
%we can evaluate the \textbf{marginalization inconsistency} by comparing the predicted marginals ${\hat{p}(y_k \mid Q_k, X)}$ to the marginals computed from the joint distribution ${\hat{p}^\mar(y_k \mid Q_k, X)}$.
%These computed marginals are obtained by integrating the joint distribution over all variables except $y_k$, i.e.,
%%
%\begin{align*}
%\hat{p}^\mar(y_k \mid Q_k, X) := \int_{\R} \hat{p}(y \mid Q, X) \, \dd{y_{-k}}
%\end{align*}
%%
%Sampling from ${\hat{p}(y_k \mid Q_k, X)}$ is trivial, but sampling from the marginal ${\hat{p}^\mar(y_k \mid Q_k, X)}$ is more challenging due to integration.
%To address this, we sample from the joint distribution ${\hat{p}(y \mid Q, X)}$ and treat the $k$-th dimension as a sample from the marginal distribution ${\hat{p}^\mar(y_k \mid Q_k, X)}$.
%%
%The marginalization inconsistency $\MI$ is then defined as the average Wasserstein distance between the predicted marginals and the computed marginals, across all variables $k$:
%%
%\begin{align}\label{eq:marginal_inconsistency}
%	\MI\bigl( \hat{p}(y \mid X, Q) \bigr) := \frac{1}{K} \sum_{k=1}^{K} \text{WD}_r \bigl( \hat{p}(y_k \mid Q_k, X), \hat{p}^\mar(y_k \mid Q_k, X) \bigr)
%\end{align}
%%
%In experiments, we set $r=2$ and approximate~\eqref{eq:marginal_inconsistency} using 1000 samples.
%%
%Currently, we only use univariate marginals to assess marginalization inconsistency. In principle, multivariate marginals could also be used, however they are computationally prohibitively expensive due to a lack of a closed form solution for the WD as in \eqref{eq:wd_empirical}.


\begin{figure*}
\centering
\small
\setlength{\tabcolsep}{2pt}%\setlength{\arraystretch}{0}
%\resizebox{0.8\linewidth}{!}{
\begin{tabular}{rcccc@{\quad}rcccc}
	& ground & \multirow{1}{*}{\MyModel(1)} & \multirow{1}{*}{ProFITi} & \multirow{1}{*}{GPR} & & ground & \multirow{1}{*}{\MyModel(4)} & \multirow{1}{*}{ProFITi} & \multirow{1}{*}{GPR} \\
	%& truth & (ours) & \citep{Yalavarthi2024.Probabilistica} & \citep{Bonilla2007.Multitask} & & truth & (ours) & \citep{Yalavarthi2024.Probabilistica} & \citep{Bonilla2007.Multitask}
	%\\
	& truth & (ours) &  &  & & truth & (ours) &  &
	\\
	& & \scriptsize $\MWD$ = 0.05 & \scriptsize $\MWD$ = 1.59 & \scriptsize $\MWD$ = 0.05 & & &\scriptsize $\MWD$ = 0.01 & \scriptsize $\MWD$ = 1.33 & \scriptsize $\MWD$ = 0.01
	\\
	\raisebox{0.5cm}{\rotatebox[origin=c]{90}{samples}}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/gt_toy_joint.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/mnf_toy_joint.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/profiti_toy_joint.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/gmix_toy_joint.pdf}
	&	\raisebox{0.5cm}{\rotatebox[origin=c]{90}{samples}}
	&	\includegraphics[width=0.09\textwidth]{fig/circle/gt_circle_joint.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/circle/mnf_circle_joint.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/circle/profiti_circle_joint.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/circle/gmix_circle_joint.pdf}
	\\	\raisebox{0.5cm}{\rotatebox[origin=c]{90}{$p(y_1)$}}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/gt_toy_y1.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/mnf_toy_y1_both.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/profiti_toy_y1_both.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/gmix_toy_y1_both.pdf}
	&	\raisebox{0.5cm}{\rotatebox[origin=c]{90}{$p(y_1)$}}
	&	\includegraphics[width=0.09\textwidth]{fig/circle/gt_circle_y1.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/circle/mnf_circle_y1_both.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/circle/profiti_circle_y1_both.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/circle/gmix_circle_y1_both.pdf}
	\\	\raisebox{0.5cm}{\rotatebox[origin=c]{90}{$p(y_2)$}}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/gt_toy_y2.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/mnf_toy_y2_both.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/profiti_toy_y2_both.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/gmix_toy_y2_both.pdf}
	&	\raisebox{0.5cm}{\rotatebox[origin=c]{90}{$p(y_2)$}}
	&	\includegraphics[width=0.09\textwidth]{fig/circle/gt_circle_y2.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/circle/mnf_circle_y2_both.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/circle/profiti_circle_y2_both.pdf}
	&	\includegraphics[width=0.09\textwidth]{fig/toy/gmix_toy_y2_both.pdf}
	\\ \multicolumn{10}{c}{\scriptsize
		\crule[teal!60!green!40]{5mm}{2mm} ground truth marginal density
		\quad\crule[red!40]{5mm}{2mm} predicted marginal density
		\quad\crule[blue!40]{5mm}{2mm} marginalized joint density
	}
\end{tabular}
%}
\caption{%
	Demonstration of marginal consistency for $\MyModel$ (ours), ProFITi~\cite{Yalavarthi2024.Probabilistica}, and Gaussian Process Regression~\cite{Bonilla2007.Multitask} on two toy datasets: blast (left) and circle (right). ProFITi is inconsistent w.r.t. the marginals of the second variable $y_2$, while $\MyModel$ is consistent with the marginals of both $y_1$ and $y_2$. $\MyModel(D)$ indicates $D$ mixture components. Gaussian Process Regression (GPR) is marginalization consistent but predicts incorrect distributions.
	%	Demonstration of marginal consistency for $\MyModel$ (ours),
	%	ProFITi~\cite{Yalavarthi2024.Probabilistica},
	%	and Gaussian Process Regression~\cite{Bonilla2007.Multitask} on two toy datasets: blast (left) and circle (right).
	%	ProFITi is inconsistent w.r.t.\ the marginals of the second variable $y_2$
	%	whereas $\MyModel$ is consistent with respect to marginals of both $y_1$ and $y_2$.
	%	$\MyModel(D)$ indicates $D$-many mixture components. Gaussian Process Regression (GPR)
	%	is consistent w.r.t.\ the marginals but predicted wrong distributions.
}%
\label{fig:spaghetti}
\end{figure*}

%We demonstrate the marginalization consistency of $\MyModel$ using two simple bivariate distributions.
%The equations to generate these distributions are provided in Appendix~\ref{sec:supp_dsets}.
%The task is unconditional density estimation.
%$\MyModel$ predicts both joints and marginals correctly, showing marginalization consistency.
%ProFITi predicts correct joints for the blast dataset and close to correct joints for the circle but is inconsistent in the marginal distribution of the second variable in both examples.
%This inconsistency arises because ProFITi uses invertible triangular attention to learn the covariance between variables, causing the second variable to always depend on the first.
%In contrast, the Gaussian Process Regression model is marginalization consistent but cannot predict correct distributions.


==> contents/abstract-lst.tex <==
\begin{abstract}
Probabilistic forecasting models for joint
distributions of targets in irregular time series are a heavily under-researched
area in machine learning with, to the best of our knowledge, only two
models researched so far:
  GPR, the Gaussian Process Regression model \citep{Durichen2015.Multitask}
    uses a multivariate normal distribution as predictive distribution, and
  ProFITi \citep{Yalavarthi2024.Profiti}
    uses a normalizing flow model based on invertible self attention layers.
While ProFITi, thanks to using normalizing flows, is the more expressive model
with a better predictive performance, we will show that it suffers from
marginal inconsistency: it does not guarantee that the marginal
distributions of a subset of variables in its predictive distributions coincide
with the directly predicted distributions of these variables.


We develop a  novel probabilistic irregular time series forecasting model,
  Marginalization Consistent Mixtures of Conditional Flows ($\MyModel$),
  that  mixes several normalizing flows with (i) Gaussians
    with full covariance matrix
  as source distributions % (but the usual identity matrix)
  and (ii) a
    separable
  invertible transformation,
    % (i.e., for each dimension separately, instead of the usual multivariate ones),
  aiming to combine the expressivity of
  normalizing flows with the marginalization consistency of mixtures of Gaussians.
%
 In experiments on four different datasets we show that
   Marginalization Consistent Mixtures of Conditional Flows outperform
   other state-of-the-art marginal consistent models, perform on par
   with ProFITi, but different from ProFITi, guarantee marginal consistency.
\end{abstract}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "../MNF-lst"
%%% End:


==> contents/background.tex <==
\section{Background}\label{sec:background}

\subsection{Density Estimation via Gaussian Mixture Model}\label{sec:mix_gaussians}

A Gaussian mixture model (GMM) with $D$-many Gaussian components
is a composite probability distribution consisting of multiple Gaussian distributions.
It estimates the joint density of variables, $y\in \R^K$, expressed as:
%
\begin{align}
\GMM(y;  w_1,\ldots,w_D, \mu_1,\ldots,\mu_D, \Sigma_1, \ldots, \Sigma_D)
	= \sum_{d=1}^{D} w_d \mathcal{N}(y;\mu_d, \Sigma_d)
\end{align}
%
Here, $\mu_d$ and $\Sigma_d$ denote the mean vector (non-negative)
and covariance matrix (symmetric positive definite) of the $d$-th Gaussian, respectively.
The weights $w_d \in [0,1]$ satisfy $\sum_{d=1}^{D} w_d = 1$.
GMM can approximate any smooth probability density
function with minimal error, provided an adequate number
of components. One can make GMMs to predict the conditional density
by parametrizing the parameters $\mu, \Sigma, w$ using the conditional input.

GMM not only marginalizes joint density
without necessitating integration but is also
marginalization consistent~\cite{}.
\todo{Cite marginalization consistency of GMMs}
However, a significant drawback of GMM lies in its
tendency to require a large number of components
to approximate even relatively simple distributions
as shown in Figure~\ref{fig:gmm}.
%This poses computational
%challenges due to the cubic complexity ($O(K^3)$)
%involved in density computation, as the square root of
%the covariance matrix, $\sqrt{\Sigma_d}$, is needed.

\begin{figure*}
	\centering
	\begin{subfigure}{0.19\textwidth}
		\includegraphics[width=0.8\textwidth]{contents/fig/demo_figs/true_dist.pdf}
		\caption{Ground truth}
	\end{subfigure}
%
	\begin{subfigure}{0.19\textwidth}
		\includegraphics[width=0.8\textwidth]{contents/fig/demo_figs/MyModel.pdf}
		\caption{$\MyModel$ (1)}
	\end{subfigure}
%
	\begin{subfigure}{0.19\textwidth}
		\includegraphics[width=0.8\textwidth]{contents/fig/demo_figs/g_mix_1.pdf}
		\caption{GMM (1)}
	\end{subfigure}
%
	\begin{subfigure}{0.19\textwidth}
		\includegraphics[width=0.8\textwidth]{contents/fig/demo_figs/g_mix_5.pdf}
		\caption{GMM (5)}
	\end{subfigure}
%
	\begin{subfigure}{0.19\textwidth}
		\includegraphics[width=0.8\textwidth]{contents/fig/demo_figs/g_mix_10.pdf}
		\caption{GMM (10)}
	\end{subfigure}
\caption{Comparison of distributions predicted by $\MyModel$ with GMM\@. $(\cdot)$ represents
	number of components. $\MyModel$ with $1$ component predicts distribution close
	to ground truth while GMM requires $10$ components.}%
\label{fig:gmm}
\end{figure*}

\subsection{Density Estimation via Normalizing Flows}\label{sec:normalizing_flows}

Normalizing flow is an unconditional density model which can
approximate any complex distribution by applying invertible transformations $f(\cdot; \theta)$,
with parameters $\theta$, on a simple base distribution $p_Z(\cdot)$ (ex.\ Gaussian)~\cite{Papamakarios2021.Normalizing,Tabak2013.Family}. Then:
%
\begin{align*}
	p_Y(y) = p_Z(f^{-1}(y; \theta))
	\cdot \left| \det \left(\pdv{f^{-1}(y;\theta)}{y}\right)\right|
\end{align*}
%
where $\pdv{y} f^{-1}(y;\theta)$ is the Jacobian of $f^{-1}(y;\theta)$ at $y$.
Normalizing flows predicts the conditional density ($p_Y(y\mid x)$) by parametrizing $f$ and
$p_Z$ with conditioning input $x$.

The base distribution $p_Z$ is often a simple distribution
like an isotropic Gaussian, and
the transformation function $f$ is multivariate and non-decomposable
allowing to learn multivariate distributions.
This makes normalizing flows more expressive than
Gaussian Mixture Models (GMMs) for modeling complex
distributions. However, being non-decomposable, the transformation
function can make it difficult to marginalize the multivariate
distribution, requiring an integral,
which is a disadvantage of normalizing flows.

\begin{comment}
Gaussian mixture model is a mixture of multiple Gaussian distributions
and predicts the unconditional joint density.
Joint density of variables $y\in \R^K$ is computed as shown below:
%
\begin{align}
	\GMM(y; \mu^1,\ldots,\mu^D, \Sigma^1, \ldots, \Sigma^D, w_1,\ldots,w_D)
	= \sum_{d=1}^{D}w_d\mathcal{N}(y;\mu^d, \Sigma^d)
\end{align}
%
$D$ is the total number of Gaussian components in GMM, $\mu^d$ and $\Sigma^d$
are the mean vector and covariance matrix of $d-\text{th}$ Gaussian, $\sum_{d=1}^{D} w_d = 1$.
Advantages of GMM are
%
\begin{enumerate}
	\item GMM can approximate any smooth probability density function with any
	specific non-zero error given enough components.
	\item Can compute the marginal densities without requiring an integral.
\end{enumerate}
%
One can make GMM to predict density of $y$ conditioned upon $x$
by parametrizing the variables from the conditioning input $x$ as shown below:
%
\begin{align}
	\GMM(y|x) = \sum_{d=1}^{D}w_d(x)\mathcal{N}(y;\mu^d(x), \Sigma^d(x))
\end{align}
%
Here, $w_d, \mu^d$ and $\Sigma^d$ are functions of $x$.

Major disadvantage of GMM is, it requires large number of
components even to approximate a simple density
function (ex.\ long tail distributions) which is computationally challenging
as computing density have cubic complexity is $K$ as
we require $\sqrt{\Sigma^d}$.
\end{comment}


==> contents/intro-lst.tex <==
\section{Introduction}\label{sec:intro}

In many real-world domains ranging from health to astronomy
time-variant data is measured in an irregular fashion:
different channels are measured at different times and usually
not on a regular grid.
Besides mere point estimates, i.e., just the
  \textbf{expected target values}
for some channels at some future time points,
one usually is interested in a probabilistic/distributional forecast of
  \textbf{a distribution of target values}.
A full predicted distribution of target values provides way more
information about the targets. For example, when bioengineers
are growing bacteria in tanks they are interested in predicting the oxygen
levels. The expected value is already interesting, but if additionally
we can predict more finegrained the whole distribution of possible
oxygen levels this allows them now to quantify the risk that the oxygen
level falls below some critical threshold and all bacteria die; the expected
value alone is not sufficient to do so.
% TODO: can we find a reference?
Consequently in recent years several models have been developed
for probabilistic forecasting irregular time series
   \citep{DeBrouwer2019.GRUODEBayes, Deng2020.Modeling, % CTFP
     Bilos2021.Neural, Schirmer2022.Modeling, Shukla2022.Heteroscedastic}.

However, all these models are limited to forecasting the distribution of
the \textbf{value of a single channel at a single time}. But decision makers require
often information about several variables and their interaction, that is,
about the predicted joint distribution of several channels at several times.
In our initial example, the bioengineers will be interested not just in the
forecasts of the oxygen levels and the biomass, but also in their interaction:
a risk for either low biomass or low oxygen levels might be tolerable,
but a risk that both occur at the same time will require their intervention.
% TODO: is there a better example?

Probabilistic forecasting models for joint
distributions of targets in irregular time series are an heavily underresearched
area in machine learning with, to the best of our knowledge, only two
models researched so far:
  GPR, the Gaussian Process Regression model \citep{Durichen2015.Multitask}
    uses a multivariate normal distribution as predictive distribution, and
  ProFITi \citep{Yalavarthi2024.Profiti}
    uses a normalizing flow model based on invertible self attention layers.
ProFITi, thanks to using normalizing flows, is able to learn way more
expressive predictive distributions, for example, it could express
multi-modal predictive distributions, while GPR being limited to multivariate
normals cannot do that. Consequently, it outperforms GPR by a wide margin
in experiments.

Models for probabilistic forecasting of joint target distributions in irregular
time series have to be able to express distributions over a varying number
of variables, as by the nature of irregular time series a forecast for say the
next 3 minutes for some training instances may involve 5 observations,
for others 7 observations. However, this capability to provide predictive distributions for
a varying number of observations/variables introduces a new issue:
to get the predictive joint distribution for values of channels at some time
points, we can query the model multiple ways:
  (i) we can just ask for the predictive distribution of those variables directly or
  (ii) we can ask for a predictive distribution of these variables plus some further
    variables and then marginalize out those additional variables again from the
    answer provided by the model.
Using a consistent model we expect to get the same answer either way.
An important special case is that the single variable marginals
of all predictive distributions provided by a model should agree with
the single variable predictive distributions it provides when we query it directly.
We call this property \textbf{marginal consistency}.

We will show in this paper that the currently best performing probabilistic
forecasting model for joint target distributions in irregular time series,
ProFITi, neither provides any guarantees to be marginal consistent nor
empirically happens to be marginal consistent on the standard datasets
used in experiments. In contrast, GPR provides guarantees for
marginal consistency, but worse predictive performance.

From this starting point we will construct a novel model that combines
the ideas of multivariate Gaussians and normalizing flows in a way
completely different from ProFITi and GPR, to achieve both,
guaranteed marginal consistency and high predictive accuracy
(see fig.~\ref{fig:}).

% TODO: remove the following paragraph, if we do not get the experiments
%   done for this aspect or it simply does not fit into the 8 pages.
%   In any case, maybe move this better to the end / discussion, as it
%   may be overcomplicated / too early here.
Moreover, at first sight our initial finding that ProFITi despite being not
marginal consistent provides a better predictive performance than
GPR might sound contra-intuitive: if GPR has a better inductive
bias, it gets the marginals at least consistent automatically,
should it then not also perform better, because it does not have to
waste data on learning marginal consistency? We will formulate another
concept, \textbf{informative queries}, that helps to explain how models
can leverage information from the queries being asked if they
violate marginal consistency. We will argue that this is a training artifact
and an unwanted behavior of the models.

Overall are our contributions as follows:
\begin{itemize}
\item
  We propose a measure for the degree of marginal consistency
  of models for joint distributions with varying size, the Wasserstein
  Distance between the (possibly numerically) marginalized predicted
  joint distribution of several variables and the directly predicted
  marginal distribution.

\item
  We show that the currently best performing model for probabilistic
  irregular time series forecasting, ProFITi, does not provide any guarantees
  for marginal consistency, and in experiments we show furthermore that
  it actually suffers from marginal inconsistency.

\item
  We develop a  novel probabilistic irregular time series forecasting model,
  Marginalization Consistent Mixtures of Conditional Flows (MarCon),
  that  mixes several normalizing flows with (i) Gaussians
    \textbf{with full covariance matrix}
  as source distributions (but the usual identity matrix)
  and (ii) a
    \textbf{separable}
  invertible transformation (i.e., for each dimension separately,
  instead of the usual multivariate ones), aiming to combine the expressivity of
  normalizing flows with the marginalization consistency of mixtures of Gaussians.

\item
  We prove that Marginalization Consistent Mixtures of Conditional Flows
  are guaranteed marginalization consistent.

\item
   In experiments on four different datasets we show that
   Marginalization Consistent Mixtures of Conditional Flows outperform
   other state-of-the-art marginal consistent models, perform on par
   with ProFITi, but different from ProFITi, guarantee marginal consistency.
\end{itemize}

Our source code can be found at~\href{}.
\todo{Add link to the source code}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "../MNF-lst"
%%% End:


==> contents/neurips_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section*{NeurIPS Paper Checklist}

\begin{enumerate}
	
	\item {\bf Claims}
	\item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
	\item[] Answer: \answerYes{}
	\item[] Justification: Please go through theorem 5.1 and Tables 1 and 2
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the abstract and introduction do not include the claims made in the paper.
		\item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
		\item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
		\item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
	\end{itemize}
	
	\item {\bf Limitations}
	\item[] Question: Does the paper discuss the limitations of the work performed by the authors?
	\item[] Answer: \answerYes{}
	\item[] Justification: Please go through Section~\ref{sec:limitations}
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
		\item The authors are encouraged to create a separate "Limitations" section in their paper.
		\item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
		\item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
		\item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
		\item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
		\item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
		\item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
	\end{itemize}
	
	\item {\bf Theory assumptions and proofs}
	\item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
	\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: Please go through Section~\ref{appendix:theory}
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the paper does not include theoretical results. 
		\item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
		\item All assumptions should be clearly stated or referenced in the statement of any theorems.
		\item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
		\item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
		\item Theorems and Lemmas that the proof relies upon should be properly referenced. 
	\end{itemize}
	
	\item {\bf Experimental result reproducibility}
	\item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
	\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: Architecture is explained in detail in Section~\ref{sec:mix_flows}. Source code was provided in Anonymous link; hyperparameter optimization protocol is given
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the paper does not include experiments.
		\item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
		\item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
		\item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
		\item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
		\begin{enumerate}
			\item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
			\item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
			\item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
			\item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
		\end{enumerate}
	\end{itemize}
	
	
	\item {\bf Open access to data and code}
	\item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
	\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: Code is given via anonymous link which will be made public. Physionet and USHCN are opensource can be easily downloaded via our code, MIMIC-III and MIMIC-IV are restrictive and require special permissions. Hence, we did not make it open access.
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that paper does not include experiments requiring code.
		\item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
		\item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
		\item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
		\item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
		\item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
		\item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
		\item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
	\end{itemize}
	
	
	\item {\bf Experimental setting/details}
	\item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
	\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: Section~\ref{sec:exp}
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the paper does not include experiments.
		\item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
		\item The full details can be provided either with the code, in appendix, or as supplemental material.
	\end{itemize}
	
	\item {\bf Experiment statistical significance}
	\item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
	\item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: \justificationTODO{}
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the paper does not include experiments.
		\item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
		\item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
		\item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
		\item The assumptions made should be given (e.g., Normally distributed errors).
		\item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
		\item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
		\item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
		\item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
	\end{itemize}
	
	\item {\bf Experiments compute resources}
	\item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
	\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: Section~\ref{sec:exp}
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the paper does not include experiments.
		\item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
		\item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
		\item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
	\end{itemize}
	
	\item {\bf Code of ethics}
	\item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
	\item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: NA
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
		\item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
		\item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
	\end{itemize}
	
	
	\item {\bf Broader impacts}
	\item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
	\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: Our research is not application oriented hence to the best of our knowledge does not have negative societal impacts
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that there is no societal impact of the work performed.
		\item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
		\item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
		\item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
		\item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
		\item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
	\end{itemize}
	
	\item {\bf Safeguards}
	\item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
	\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: \answerNA{}
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the paper poses no such risks.
		\item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
		\item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
		\item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
	\end{itemize}
	
	\item {\bf Licenses for existing assets}
	\item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
	\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: \answerNA{}
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the paper does not use existing assets.
		\item The authors should cite the original paper that produced the code package or dataset.
		\item The authors should state which version of the asset is used and, if possible, include a URL.
		\item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
		\item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
		\item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
		\item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
		\item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
	\end{itemize}
	
	\item {\bf New assets}
	\item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
	\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: \answerNA{}
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the paper does not release new assets.
		\item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
		\item The paper should discuss whether and how consent was obtained from people whose asset is used.
		\item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
	\end{itemize}
	
	\item {\bf Crowdsourcing and research with human subjects}
	\item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
	\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: \answerNA{}
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
		\item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
		\item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
	\end{itemize}
	
	\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
	\item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
	\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: \answerNA{}
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
		\item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
		\item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
		\item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
	\end{itemize}
	
	\item {\bf Declaration of LLM usage}
	\item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
	%this research? 
	\item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
	\item[] Justification: \answerNA{}
	\item[] Guidelines:
	\begin{itemize}
		\item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
		\item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
	\end{itemize}
	
\end{enumerate}

==> contents/prop_model-lst.tex <==
\section{Constructing Marginal Consistent Conditional Distributions}\label{sec:mc_layers}

We look for conditional distributions $p(y_1,\ldots,y_K \mid x^\qry_1,\ldots,x^\qry_K, x^\ctx)$,
where each $x^\qry_k$ is
  the condition for each corresponding $y_k$ only, but
  not for any other $y_{k'}$ ($k'\neq k$),
  and additionally all $y_k$ can depend on a common $x^\ctx$.
Technically, one can capture this intuitive concept by requiring
the distribution to be jointly permutation invariant in $x^\qry, y$ \citep{Yalavarthi2024.Profiti}.
% TODO: check the profiti paper and add this sentence and maybe an example there.
For simplicity, we assume univariate $y_k\in\R$, but cover multivariate $x^\qry_k\in\R^L$
and $x^\ctx\in\R^{L^\ctx}$.

\paragraph{Separably parametrized Gaussians.}
The arguably most simple
  conditional
  permutation invariant
  distribution for variably many variables
is a multivariate Gaussian ${\cal N}(y \mid \mu(x), \Sigma(x))$ who's
  conditional mean function $\mu(x)$ and
  conditional covariance function $\Sigma(x)$
are separable, i.e.,
%
\begin{align*}
  \mu(x)_k & := \tilde\mu(x^\qry_k, x^\ctx)
\\ \Sigma(x)_{k,\ell} &:= \tilde \Sigma(x^\qry_k, x^\qry_{\ell}, x^\ctx)
\end{align*}
for a mean function $\tilde\mu:\R^L\times\R^{L^\ctx}\rightarrow\R$ and
a covariance function $\tilde\Sigma:\R^L\times\R^L\times\R^{L^\ctx}\rightarrow\R$,
a setup very well known from Gaussian processes.
Such a separably parametrized multivariate Gaussian
also is marginal consistent.

\begin{lemma}
Any conditional multivariate Gaussian ${\cal N}(y \mid \mu(x), \Sigma(x))$
  with separable conditional mean function $\mu(x)$ and
  separable conditional covariance function $\Sigma(x)$
is marginal consistent.
\end{lemma}
% TODO: add proof to the appendix and a reference here.

\paragraph{Separable Normalizing Flows.}

% TODO: we need to rewrite this for conditional distributions.
% "marginal consistent" is a only useful for conditional distributions.

Normalizing flows model distributions by transforming a
source distribution $p_Z$ on $\R^K$
by means of an invertible transformation $f: \R^K\rightarrow\R^K$.
Then the target distribution, the distribution of the image of $f$ can
be concisely described by the Jacobian of the inverse transformation:
%
\begin{align*}
	p_Y(y) := p_Z(f^{-1}(y; \theta))
	\cdot \left| \det \left(\pdv{f^{-1}(y;\theta)}{y}\right)\right|
\end{align*}
%
Existing approaches to normalizing flows use very simple source distributions,
typically a multivariate standard normal $p_Z(z):={\cal N}_K(z \mid 0_K, 1_{K\times K})$,
and model interactions between variables by means of the transformation
$f$.
% TODO: cite 3-4 such approaches.
Current approaches for conditional normalizing flows for varying number of variables
followed the same approach and tackled the problem by engineering
expressive transformations between vectors of same size, for any size
   \citep{Liu2019.Graph, % GNF
	      Bilos2021.Normalizing,  % SNF
              Yalavarthi2024.Profiti}.
%    \citep{Satorras2021.Equivarianta} % E(N) -- not a NF; uses a GNN
For example, ProFITi, uses an invertible attention mechanism.

All these models in general will not have a guarantee for marginal
consistency. To the best of our knowledge there is no light condition on
the transform that would provide such a guarantee.

We therefore propose a drastic change, reversing the standard approach
for normalizing flows: to combine
  (i) simple, separable transforms with
  (ii) a richer source distribution, Gaussians with full covariance matrix.
This way interactions between variables cannot be represented by
the transform anymore, but they can be represented by the covariance
of the source distribution. The resulting normalizing flow is marginal consistent.

\begin{lemma}\label{lemma:separable_flows}
Any conditional  normalizing flow $p_Y$ with
(i)  a marginal consistent source distribution $p_Z$ and
(ii) a separable transformation
      $f(z \mid x^\qry, x^\ctx):= (\phi(z_1 \mid x_1^\qry, x^\ctx),\ldots,\phi(z_K \mid x_K^\qry, x^\ctx))$
  (for $z\in\R^K, x^\qry\in\R^{K\times L}$)
  for some function $g:\R\times\R^L\times\R^{L^\ctx}\rightarrow\R$
    that is invertible in its first argument
is marginal consistent.
\end{lemma}
% TODO: add proof to the appendix and a reference here.

\paragraph{Commonly weighted Mixtures.}
When using separably parametrized Gaussians as source distributions in
Lemma~\ref{lemma:separable_flows} and expressive univariate transformations,
we can model any kind of marginal as well as rich interactions between variables.
However, the model is still restricted with respect to modality: due to the unimodality
of the Gaussian and the variable-wise separable transformations,
it will always be unimodal itself. We therefore
resort to the most simple way to achieve multimodality: we combine
several of such separable flows into a mixture model. When using
mixture weights that do not depend on the component conditioners $x_k$ at
all, but just by the common conditioner $x^\ctx$, the model stays marginal consistent.

\begin{lemma}\label{lemma:separable_flows}
Any conditional mixture model $p_Y$
%
\begin{align*}
  p_Y(y \mid x^\qry, x^\ctx) := \sum_{d=1}^D w_d(x^\ctx) \, p^{\text{comp}}_d(y \mid x^\qry, x^\ctx)
\end{align*}
%
with
(i)  a marginal consistent component models $p^{\text{comp}}_d$ and
(ii) a conditional weight function $w: \R^{L^\ctx}\rightarrow\R^D$
  that depends only on the common conditioners,
is marginal consistent.
\end{lemma}
% TODO: add proof to the appendix and a reference here.



\section{Mixtures of Separable Flows}\label{sec:mix_flows}
Based on the constructions from the last section, we propose to build
a marginal consistent model for forecasting irregular time series in
four components (see fig.~\ref{fig:propmodel}):
\begin{enumerate}
\item a separable encoder, delivering
  \\ (i) an encoding $h^\ctx:= \text{enc}^\ctx(x^\obs)$ of the observations, used for all queries,
         and
  \\ (ii) $D$ encodings $h^\qry_{d,k}:=\text{enc}(x^\qry_k, h^\ctx; \theta^{\text{enc}}_d)$
     of each query.
% TODO: do we really want to use h^\qry and no just h ? this introduces a lot of clutter.
%     otherwise the distinction between h^\ctx and h is not very explicit.
\item $D$ Gaussian source distributions $p^{\text{src}}_d(z \mid \mu_d, \Sigma_d)$,
   \\ each separably parametrized by the encoded queries $h^\qry_d$.
\item $D$ separable normalizing flows $\hat{p}^\flow_d$,
    one on top of each of the source distributions,
    \\ also separably parametrized by the encoded queries $\hs_d^\qry_d$.

\item a mixture $\hat p(y \mid w)$ of the $D$ normalizing flows with mixing weights
    $w:= w(h^\ctx)$
  \\ depending only on the encoded observations $h^\ctx$, but not the queries.
\end{enumerate}


\paragraph{1. Separable Encoder.}
%  $h_k := \text{enc}(x^\qry_k, x^\ctx; \theta^{\text{enc}}) $
% TODO: reference tripletformer.
To encode the
  past observations $x^\obs:= (t^\obs_n, c^\obs_n, v^\obs_n)_{n=1:N}$ and
  queries $x^\qry:= (t^\qry_k, c^\qry_k)_{k=1:K}$ we use a
  positional embedding
  \begin{align*}
	\posembed(t)_ m := \begin{cases}
		a_{m}t + b_m & \text{if } m = 1 \\
		\sin(a_{m}t + b_m) & \text{else}
	\end{cases}
  \end{align*}
with learnable parameters $a_m, b_m$ for the time and
one-hot encodings for the channel:
\begin{align*}
   \tilde x^\ctx_n & := [ \posembed(t^\obs_n), \onehot(c^\obs_n), v^\obs_n ]_{n=1:N} \\
   \tilde x^\qry_n   & := [ \posembed(t^\qry_k), \onehot(c^\qry_k) ]_{k=1:K}
\end{align*}
The observations are further encoded via self attention and the queries via
cross attention w.r.t.\ the (encoded) observations:
\begin{align*}
    h^\ctx &:= \mha(\tilde x^\ctx, \tilde x^\ctx, \tilde x^\ctx; \theta^{\text{enc-com}}) \\
    h^\qry     &:= \mha(\tilde x^\qry, h^\ctx, h^\ctx; \theta^{\text{enc-qu}}) \\
\end{align*}
For the encoding of the queries we use an encoding dimension $DM$ and reshape each
$h^\qry_k$ into $D$ encodings $h^\qry_{d,k}$ of dimension $M$.




\paragraph{2. $D$ separably parametrized Gaussian source distributions
  $p^{\text{src}}_d(z \mid \mu_d, \Sigma_d)$.}
We model means and covariances simply by a linear and a quadratic function
in the encoded queries $h_d$:
\begin{subequations}\label{eq:mu_sigma_func}
\begin{align}
	\label{eq:mu_func}
	\mu(\hs_d) &= \hs_d \theta^\mean
	&&\implies& \mu(\hs_d)_k &=  \hs_{d,k}\theta^\mean \, \quad 1\le k\le K
	\\ \label{eq:sigma_func}
	\Sigma(\hs_d) &= \frac{\hs_d \theta^\cov (\hs_d \theta^\cov)^T}{\sqrt{M'}} + \bI_K
	&&\implies& \Sigma(\hs_d)_{k,l} &= \frac{\hs_{d,k} \theta^\cov (\hs_{d,l} \theta^\cov)^T}{\sqrt{M'}} + \delta_{kl} \quad 1\le k,l \le K
\end{align}
\end{subequations}
%
where $\theta^\mean \in \R^{M\times 1}$ and $\theta^\cov \in \R^{M\times M'}$
are trainable weights; $\bI_K$ is an identity matrix of size $K$, and
$\delta_{kl} = 1$ if $k=l$ else $0$.
In~\eqref{eq:sigma_func}, we divide the inner product with $\sqrt{M'}$
for stable learning as done in~\cite{Vaswani2017.Attention}.
$\Sigma(\hs_d)$ is guaranteed to be positive definite.
%
\begin{lemma}
	$\Sigma(\hs_d)$ is always a positive definite matrix.
\end{lemma}
\begin{proof}
	Sum of a positive semi-definite matrix (ex.\ $\frac{\hs_d \theta^\cov (\hs_d \theta^\cov)^T}{\sqrt{M'}}$) and positive definite matrix (ex. $\bI_K$) is always positive definite.
\end{proof}
%
When calculating the density of a multivariate Gaussian (our source distribution),
in practice, $\Sigma^{\frac{1}{2}}$ is sufficient rather than $\Sigma$.
However, since the decomposition of a Gaussian distribution
is performed using $\Sigma$, parameterizing $\Sigma^{\frac{1}{2}}$
does not satisfy~\ref{con:cov}, thus violating the consistency.
%Hence, we parametrize $\Sigma$.


\paragraph{3. $D$ separable normalizing flows $\hat{p}_d^\flow$.}
TODO

\paragraph{4. Mixture Model.}
We model the mixture weights via cross attention,
using trainable parameters $\beta\in \R^{D\times M}$ as attention queries
and a softmax to ensure the weights to sum to $1$:
\begin{align*}
	w := \softmax(\mha(\beta, h^\obs, h^\obs; \theta^\mix))
\end{align*}





\newpage



\begin{figure}
	\centering
	\import{fig/tikzpictures}{model_arch}
	\caption{Illustration of proposed $\MyModel$.
		$D$-many flows (fixed). $K$-many variables (variable).
		Encoder (enc) takes $\X, \Q$ (observed series and query timepoint-channel ids.; conditioners) as input, and outputs
	an embedding $x$ and $w$. $\mu, \Sigma$ of $p_{Z_d}$ are
	parametrized by $\hs_d$.  Flow transformation of $p_{Z_d}$ is parametrized
	by $\hs_d$. Transformation layer consists of $K$-many univariate
	transformations $\phi$. $\phi$ that
	transforms $z_k$ of $z\sim p_{Z_d}(z\mid x)$ is parametrized by $\hs_{d,k}$.
	}\label{fig:propmodel}
\end{figure}

Predicting marginal distributions of normalizing flows is
challenging when the transformation function is non-separable.
On the other hand, having a separable transformation function
does not yield multivariate distributions since the base distribution
has diagonal covariance.
To achieve both marginalization and multivariate distributions,
we can reverse the approach.
We can start with a multivariate base distribution
(allowing for dependencies between variables)
and then apply a separable transformation function.
However, a single multivariate distribution might not be
flexible enough to capture all the complexities of real-world data.
Inspired by Gaussian mixture models,
we can combine multiple ($D$ in total) normalizing flows.
Each flow would represent a different component
of the data distribution. We weight these flows
using a set of weights, $w=(w_1, \ldots, w_D)$,
where $w \in [0,1]^D, \; \sum_{d=1}^{D} w_d = 1$.
This approach allows for more expressive modeling of complex data distributions.
%
\begin{align}
	p_Y(y\mid \Q, \X)	&:= \sum_{d=1}^{D} w_d \ p_{Y_d}(y\mid \Q, \X)
	%\\	&:= \sum_{d=1}^{D} w_d p_{Z_d}({f_d}^{-1}(y; x,\theta)|x)\left|
	% \det \left(\pdv{{f^d}^{-1}(y;x,\theta)}{y}\right)\right|
\end{align}
%
The conditioners $\X$ and $\Q$ are sequence of tuples,
and one needs to encode them \emph{properly} to accommodate
varying number of variables $K$ and fixed number of components $D$
of the conditional flows.
Assume $\hs$ as the encoded information of both $\X$ and $\Q$; and act
as conditioning input in flows.
Since the transformation function is separable, $\hs$ should also be separable
meaning $\hs$ should have $K$-many inner encodings.
Additionally, a different encoding for different mixture component
allows to learn different parts of the distributions.
Hence, our $\hs\in \R^{D\times K\times M}$ where
$M$ is a latent embedding dimension.

Now $p_{Y_d}(y\mid \Q, \X)$ is equivalent to $p_{Y_d}(y\mid \hs_d)$ where:
%
\begin{align}\label{eq:mnf_formula}
	p_{Y_d}(y\mid \hs_d) = p_{Z_d}(f^{-1}(y; \hs_d, \theta)\mid \hs_d)
	\cdot \left| \det \left(\pdv{f^{-1}(y;\hs_d, \theta)}{y}\right)\right|
\end{align}
%
As mentioned in Section~\ref{sec:prilims}, marginal distribution of
$y_k$ should depend on all $\X$ and only $\Q_k$. Hence,
$\hs_{:,k,:}$ is computed from $\X$ and $\Q_k$.
Additionally, mixture weights $w$ should not depend on $\Q$ because
the number of components $D$ is fixed and making it dependent on $\Q$
would violate the marginalization consistency as different $\Q$ yields
different $w$ for same $\X$. However, we do not get this problem
if $w$ depends on $\X$.

In the following, first we discuss the major flow components
(base distribution: $p_Z$, transformation function: $f$)
and later encoder architecture to compute $\hs$ and mixture weights $w$.

\subsection{Base distribution}\label{sec:base_dist}

%The joint distributions can be achieved by the mixture of marginals as well,
%however, for better expressiveness we make the base distribution to be
%a multivariate distribution with non-diagonal covariance.

The primary choice among distributions that
require marginalization is multivariate Gaussian.
Base distribution of $d-\text{th}$ component is
$p_{Z_d} := \mathcal{N}(\mu(\hs_d), \Sigma(\hs_d))$
mean vector $\mu(\cdot)$ and covariance matrix $\Sigma(\cdot)$
are the functions of the conditioning input $\hs_d$.
\emph{Marginal distributions are calculated
by isolating the relevant rows
and columns of the covariance matrix $\Sigma(\hs_d)$ and the
corresponding elements of the mean vector $\mu(\hs_d)$.}
Hence, to be marginal consistent, we need to satisfy two constraints:
%
\begin{description}
	\item[C1\label{con:mean}] $\mu(\hs_d)_k$ is a function of $\X$ and $\Q_k$ only
	%
	\item[C2\label{con:cov}] $\Sigma(\hs_d)_{k,l}$ is a function of $\X$, $\Q_k$ and $\Q_l$ only
\end{description}
%
\begin{subequations}\label{eq:mu_sigma_func}
\begin{align}
	\label{eq:mu_func}
	\mu(\hs_d) &= \hs_d \theta^\mean
	&&\implies& \mu(\hs_d)_k &=  \hs_{d,k}\theta^\mean \, \quad 1\le k\le K
	\\ \label{eq:sigma_func}
	\Sigma(\hs_d) &= \frac{\hs_d \theta^\cov (\hs_d \theta^\cov)^T}{\sqrt{M'}} + \bI_K
	&&\implies& \Sigma(\hs_d)_{k,l} &= \frac{\hs_{d,k} \theta^\cov (\hs_{d,l} \theta^\cov)^T}{\sqrt{M'}} + \delta_{kl} \quad 1\le k,l \le K
\end{align}
\end{subequations}
%
where $\theta^\mean \in \R^{M\times 1}$ and $\theta^\cov \in \R^{M\times M'}$
are trainable weights; $\bI_K$ is an identity matrix of size $K$, and
$\delta_{kl} = 1$ if $k=l$ else $0$.
In Eq.~\eqref{eq:sigma_func}, we divide the inner product with $\sqrt{M'}$
for stable learning as done in~\cite{Vaswani2017.Attention}.
$\Sigma(\hs_d)$ is guaranteed to be positive definite.
%
\begin{lemma}
	$\Sigma(\hs_d)$ is always a positive definite matrix.
\end{lemma}
\begin{proof}
	Sum of a positive semi-definite matrix (ex.\ $\frac{\hs_d \theta^\cov (\hs_d \theta^\cov)^T}{\sqrt{M'}}$) and positive definite matrix (ex. $\bI_K$) is always positive definite.
\end{proof}
%
When calculating the density of a multivariate Gaussian (our base distribution),
in practice, $\Sigma^{\frac{1}{2}}$ is sufficient rather than $\Sigma$.
However, since the decomposition of a Gaussian distribution
is performed using $\Sigma$, parameterizing $\Sigma^{\frac{1}{2}}$
does not satisfy~\ref{con:cov}, thus violating the consistency.
%Hence, we parametrize $\Sigma$.

\subsection{Conditional univariate transformations}\label{sec:splines}

To achieve separable invertible transformations, any univariate bijective functions
can be applied on each variable separately.
Spline based functions~\cite{Durkan2019.Neural}
attracted interest due to their expressive and generalization capabilities.
We employ computationally efficient Linear Rational Spline (LRS)
transformations~\cite{Dolatabadi2020.Invertible}.
Formally, given a set of monotonically increasing points ${\{(u_m, v_m)\}_{m=1:M}}$ called knots, that is ${u_m<u_{m+1}}$ and ${v_m<v_{m+1}}$, along with their corresponding derivatives ${\{\Delta_m > 0\}_{m=1:M}}$, then the LRS transformation $\phi(u)$ within a bin $u \in [u_m, u_{m+1}]$ is:
%
\begin{align}\label{eq:lrs}
	\phi(u) =
\begin{cases}
	\frac{%
		\alpha_m v_m(\lambda_m - \tilde{u}) + \bar{\alpha}_m \bar{v}_m\tilde{u}
	}{%
		\alpha_m(\lambda_m-\tilde{u}) + \bar{\alpha}_m\tilde{u}
	} \hfill:& 0 \le \tilde{u} \le \lambda_m
	\\[1ex]
	\frac{%
		\bar{\alpha}_m \bar{v}_m(1-\tilde{u}) + \alpha_{m+1}v_{m+1}(\tilde{u} - \lambda_m)
	}{%
		\bar{\alpha}_m(1-\tilde{u}) + \alpha_{m+1}(\tilde{u} - \lambda_m)
	} \hfill:& \lambda_m \le \tilde{u} \le 1
\end{cases}
\qq{where}
\tilde{u} = \frac{u - u_m}{u_{m+1} - u_m} \in [0, 1]
\end{align}
%
Here, $\lambda_m\in(0,1)$ signifies the location of automatically inserted virtual knot between $u_m$ and $u_{m+1}$ with value $\bar{v}_m$. The values of $\lambda_m$, $\alpha_m$, $\bar{\alpha}_m$ and $\bar{v}_m$ are all automatically derived from the original knots and their derivatives~\cite{Dolatabadi2020.Invertible}.
For a conditional LRS $\phi(z_k; \hs_{d,k}, \theta)$,
the function parameters such as width and height of each bin,
the derivatives at the knots, and $\lambda$ are computed from the conditioning input
$\hs_{d,k}$ and some model parameters $\theta$. $\theta$ helps to project $\hs_{d,k}$
to the function parameters, and is common to all the variables $z_{1:K}$ so that
the transformation $\phi$ can be applied for varying number of variables $K$.
Additionally, we set $\theta$ common to all the components as well.
Since, each component
has separate embedding for a variable $z_k$ ($\hs_{d,k}$),
we achieve different transformations
in different components for same variable.

In summary, the conditional flow model is separable across the query size $f = f_1 \times \cdots \times f_K$ with
%
\begin{align}\label{eq:mnf_flow}
	f(y\mid \hs_d) &= \left(\phi(y_1, \hs_{d,1}), \ldots, \phi(y_K, \hs_{d,K})\right)
\end{align}
%


\subsection{Encoder for conditioners and mixture weights}\label{sec:enc}

\begin{wrapfigure}{r}{0.49\textwidth}
	\centering
	\small
	\import{fig/tikzpictures}{encoder}
	\captionof{figure}{Encoding conditioners. We compute $x$
		from both $\X$ and $\Q$; $w$ from $\X$ only.
	}\label{fig:encoder}
\end{wrapfigure}
%
We require an encoder that encodes $\X$ and $\Q$ together
into $\hs \in \R^{D\times K\times M}$ and $w$,
ensuring $\hs_{:,k,:}$ is derived solely
from $\X$ and $\Q_k$. For this, any model that additionally satisfy~\ref{req:permutation_invariance}
can be used.
We modify the existing state-of-the-art probabilistic interpolation model:
Tripletformer~\cite{Yalavarthi2023.Tripletformer} and use it as our encoder.

First, we convert a triplet $\X_n=(t^\obs_n, c^\obs_n, v^\obs_n)$,
and pair $\Q_k=(t^\qry_k, c^\qry_k)$ into two vectors:
%
\begin{align*}
	\xs_n &:= [\posembed(t^\obs_n), \onehot(c^\obs_n), v^\obs_n] \\
	\qs_k &:= [\posembed(t^\qry_k), \onehot(c^\qry_k)]
\end{align*}
%
Here, $\onehot$ indicates one-hot encoding and $\posembed$ is the
learned sinusoidal positional embedding given as follows:
%
\begin{align*}
	\posembed(t)[m] := \begin{cases}
		a_{m}t + b_m &; m = 1 \\
		\sin(a_{m}t + b_m) &; m>1
	\end{cases}
\end{align*}
%
where $a_m$ and $b_m$ are trainable parameters.
Multihead attention block~\cite{Vaswani2017.Attention} with $H$-many heads is given as
$\mha_H(\text{q}, \text{k}, \text{v}; \theta^\text{MHA})$ where
q, k, v indicates attention queries, attention keys and attention values respectively, and $\theta^\text{MHA}$ are trainable parameters.
We use one layer of self multihead attention
on $\xs$ and get $\hs^\obs$:
%
\begin{align}\label{eq:mha_obs}
	\hs^\obs := \mha_H(\xs, \xs, \xs; \theta^\obs)
\end{align}
%
The embedding for $\Q$ is computed by applying a
cross multihead attention between $\qs$ and $\hs^\obs$:
%
\begin{align}\label{eq:mha_query}
	\widetilde{\hs} := \mha_H(\qs, \hs^\obs, \hs^\obs; \theta^\qry) \in \R^{K\times DM}
\end{align}
%
We unstack $\widetilde{\hs}$ across the last axis and obtain the latent codes
$\hs \in \R^{D\times K\times M}$, that contain both query and observation information.


We use $\hs^\obs$ to compute the weights $w$ of the mixture components. For this,
we have $\beta\in \R^{D\times M}$ as the trainable parameters that are passed as
the attention queries. Here $\beta_d$ is used to predict $w_d$.


Then mixture weights are computed using:
%
\begin{align*}
	w := \softmax(\mha_H(\beta, \hs^\obs, \hs^\obs; \theta^\mix))
\end{align*}
%
Softmax function is used after the multihead attention to
make sum of the component weights to $1$.
Encoder architecture is demonstrated in Figure~\ref{fig:encoder}.

%Using attention mechanism to encode the conditioners
%allows us to achieve \textbf{R3}.
%More details on permutation invariance of $\MyModel$ is discussed in
%Supp.~\ref{sec:permutation_invariance}.

\subsection{Training and sampling}\label{sec:training}

Given $\mathcal{D}$, a batch of queries and answers, where
for each sample, we have $\X$, $\Q$ and $y$, we minimize
the normalized joint negative log-likelihood (njNLL)
%
\begin{align}
	\mathcal{L} = \frac{1}{|\mathcal{D}|} \sum_{(\X, \Q, y)\in \mathcal{D}} -\frac{1}{|y|}
	\log p_Y(y\mid \Q, \X)
\end{align}
%
with respect to the parameters of $\enc$, $\mu$, $\Sigma$ and $f$.

Forward pass of $\MyModel$ is provided in Algorithm~\ref{alg:fwd_pass}.
First, embedding and component weights are computed (line 1).
For every $d$, we inverse-transform $y$ and compute $z$. Using
Eq.~\eqref{eq:cvf}, we compute $p_{Y_d}(y)$ (lines 3--6).
Finally, we add all the densities using mixture weights (line 7)
to obtain $p_{Y}(y\mid \Q, \X)$ and train it for
normalized joint log likelihood loss.
For sampling $\MyModel$, we follow Algorithm~\ref{alg:inv_pass}.
After computing $x$ and $w$, we sample $d$ with the probability of $w_d$.
We transform $z$ drawn from base distribution of $d^\text{th}$
component to $y$.


\begin{theorem}\label{thm:marginal_consistency}
$\MyModel$ is marginally consistent.

\begin{proof}
	We can simply use
\end{proof}

\begin{proof}
We need to show that $\MyModel$ satisfies Equation~\eqref{eq:mar_consistency}.

First, consider the marginal query $\Q_{-k}$. Then:
%
\begin{align*}
	\hat{p}(y\mid \Q, \X)
	&= \sum_{d=1}^{D} w_d p_{Y_d}(y_{-k}\mid \Q_{-k}, \X)
\\	&= \sum_{d=1}^{D} w_d p_{Z_d}(f^{-1}(y_{-k})\mid \Q_{-k}, \X)\cdot |\det\mathbf{D}f^{-1}(y_{-k}) |
\end{align*}
%
On the  other hand, marginalizing $\MyModel(\Q, \X)$ over $y_k$ can be solved analytically:
%
\begin{align*}
	\hat{p}^\mar(y_{-k}) &= \int \hat{p}(y\mid \Q, \X) \dd{y_k}
\\	&= \int \sum_{d=1}^{D} w_d p_{Y_d}(y \mid \Q, \X) \dd{y_k}
\\	&= \sum_{d=1}^{D} w_d \int p_{Y_d}(y \mid \Q, \X) \dd{y_k}
\\	&= \sum_{d=1}^{D} w_d \int p_{Z_d}(f^{-1}(y) \mid \Q, \X) \cdot |\det \mathbf{D}f^{-1}(y_{-k})|\dd{y_k}
\end{align*}
%
Here, note that since $f$ is separable, i.e. $f = f_1\times \cdots \times f_K$, we have $f^{-1}(y) = (f_1^{-1}(y_1), \ldots, f_K^{-1}(y_K))$. In particular
%
\begin{align*}
	|\det \mathbf{D}f^{-1}(y_{-k})|
	&= |\det \diag\bigl((\mathbf{D}f_k^{-1}(y_k))_{k=1:K}\bigr)|
	= \prod_{k=1}^K |\mathbf{D}f_k^{-1}(y_k)|
% \\	&= \prod_{k=1}^K \frac{1}{|f_k'(f_k^{-1}(y_k))|}
\end{align*}
%
And secondly
%
\begin{align*}
	p_{Y_d}(y \mid \Q, \X)
\\	&= p_{Z_d}(f^{-1}(y)\mid \Q, \X)\cdot |\det\mathbf{D}f^{-1}(y) |
\\	&= p_{Z_d}((f_1\times \cdots \times f_K)^{-1}()y\mid \Q, \X)\cdot |\det\mathbf{D}f^{-1}(y) |
\end{align*}
%
\end{proof}
\end{theorem}




\begin{algorithm}[t]
\caption{Density estimation with $\MyModel$}\label{alg:fwd_pass}
\begin{algorithmic}
	\REQUIRE{$D$, $\enc(\cdot, \cdot)$, $\mu(\cdot)$, $\Sigma(\cdot)$, $\Theta(\cdot)$}
	\INPUT{$\Q, \X, y$}
	\OUTPUT{$p(y\mid \Q, \X)$}
	\STATE {$x,w \gets \enc(\Q, \X)$ \hfill $\rhd x\in \R^{D\times K\times M}$, $w \in [0,1]^D$}
	\FOR{$d \in {1, \ldots, D}$}
	\STATE {$z \gets \Flow^{-1}(y \mid \hs_d)$ \hfill $\rhd$ transform $z$ to $y$}
	\STATE {$z' \gets \pdv{y} \Flow^{-1}(y \mid \hs_d)$ \hfill $\rhd$ compute the Jacobian}
	\STATE $p_{Z_d}(z\mid \hs_d) \gets \mathcal{N}(z; \mu(\hs_d), \Sigma(\hs_d))$ \hfill $\rhd$ density of $z$
	\STATE $p_{Y_d}(y\mid \hs_d) \gets p_{Z_d}(z\mid \hs_d)\cdot |\det(z')|$ \hfill $\rhd$ density of $y$
	\ENDFOR
	\RETURN $\sum_{d=1}^{D} w_d p_{Y_d}(y\mid \hs_d)$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\caption{Sampling of $\MyModel$}%
\label{alg:inv_pass}
\begin{algorithmic}
	\REQUIRE{$D$, $\enc(\cdot, \cdot)$, $\mu(\cdot)$, $\Sigma(\cdot)$, $\Theta(\cdot)$}
	\INPUT{$\Q, \X$}
	\STATE {$\hs, w \gets \enc(\Q, \X)$ \hfill $\rhd h\in \R^{D\times K\times M}$, $w \in [0,1]^D$}
	\STATE $d \sim \text{Multinouli}(w_1, \ldots, w_D)$ \hfill $\rhd$ sample the component ID\@.
	\STATE $z\sim\mathcal{N}(\mu(\hs_d), \Sigma(\hs_d))$ \hfill $\rhd$ sample $z$
	\STATE $y \gets \Flow(z;\Theta(\hs_d))$	\hfill $\rhd$ compute $y$

	\RETURN $y$
\end{algorithmic}
\end{algorithm}

